Hierarchical Block Low-rank Approximation of Cavity Radiation

In this paper we examine the use of low-rank approximations for the handling of radiation boundary conditions in a transient heat equation given a cavity radiation setting. The finite element discretization that arises from cavity radiation is well known to be dense, which poses difficulties for efficiency and scalability of solvers. Here we consider a special treatment of the cavity radiation discretization using a block low-rank approximation combined with hierarchical matrices. We provide an overview of the methodology and discusses techniques that can be used to improve efficiency within the framework of hierarchical matrices, including the usage of the approximate cross approximation (ACA) method. We provide a number of numerical results that demonstrate the accuracy and efficiency of the approach in practical problems, and demonstrate significant speedup and memory reduction compared to the more conventional "dense matrix" approach.

==> Makefile <==
FILENAME := main

# Notes:
# 1.) To build this on an older LaTeX installation (Ubuntu 2018) I
# had to change version in the following line:
# \pgfplotsset{compat=1.18} % avoid warnings about unsuitable tick labels, missing features
# to 1.15 instead.
# 2.) There is an error about \affiliation being an undefined control sequence. I fixed
# this by generating my own elsarticle.cls file in the paper directory by running
# latex elsarticle.ins
# This seemed to fix the issue
$(FILENAME).pdf: $(FILENAME).tex references.bib
	latexmk -g -pdf $<

clean:
	latexmk -C
	rm -f *~ .*~


==> codes/HierarchicalDecomp.tex <==
\begin{algorithm}[t]
\caption{\texttt{HierarchicalDecomp}($F, T$)}\label{alg:hierarchical}

\begin{algorithmic}
\Ensure $F$ view-factor matrix and $T$ index tree
\State $\tilde{F} \gets \emptyset$  
\Comment{hierarchical matrix}
\If{ $F$ is ``large''}
    \State $[B_{00}, B_{01}; B_{10}, B_{11}] \gets F$
    \Comment{split with respect to $T$}
    \ForEach{$B \in F$}
    \If{$B$ is data sparse}
        \State $\tilde{B} \approx B$
        \Comment{low-rank approximation}
    \Else
        \State $\tilde{B} \gets $ \texttt{HierachicalDecomp}($B, T_B$)
    \Comment{recursion}
    \EndIf
    \State $\tilde{F} \gets \tilde{F} \uplus \tilde{B}$
    \EndFor
\Else 
    \State $\tilde{F} \gets F$
\EndIf
\end{algorithmic}
\end{algorithm}

==> codes/PartitionTree.tex <==
\begin{algorithm}[t]
\caption{\texttt{PartitionTree}($\vec{N}$)}\label{alg:kdtree}

\begin{algorithmic}
\Ensure $\vec{N}$ the centroids of all mesh cells in $\mathcal{M}$
\State $T \gets \emptyset$ 
\Comment{$k$-d tree}
\If{ $\vec{N}$ `large'}
    \State $[\vec{N}_{left}, \vec{N}_{right}] \gets \vec{N}$
    \Comment{split using a hyperplane}
    \State $T_{left} \gets$ \texttt{PartitionTree}$(\vec{N}_{left})$
    \State $T_{right} \gets$ \texttt{PartitionTree}$(\vec{N}_{right})$
    \State $T \gets T_{left} \uplus T_{right}$
    \Comment{left and right children}
\Else 
    \State $T \gets \vec{N}$
\EndIf
\end{algorithmic}
\end{algorithm}

==> codes/blockLU.tex <==
\begin{algorithm}[t]
\caption{\texttt{BlockLU}($A$)}\label{alg:LU}

\begin{algorithmic}
\Ensure $C$ a reflection matrix and $T$ index tree
\State $L, U \gets \emptyset$  
\Comment{hierarchical matrices}
\If{ $C$ leaf in $T$}
    \State $[L, U] \gets \texttt{LU}(C)$
    \Comment{standard LU decomposition}
\Else 
    \State $[C_{00}, C_{01}; C_{10}, C_{11}] \gets C$
    \Comment{with respect to $T$}
    \State $[L_{00}, U_{00}] \gets $ \texttt{BlockLU}($C_{00}$)
    \State $U_{01} \gets $ \texttt{BlockForwardSubst}($L_{00}, C_{01}$)
    \State $L_{10} \gets $ \texttt{BlockBackwardSubst}($U_{00}, C_{10}$)
    \State $L_{11}, U_{11} \gets $ \texttt{BlockLU}($C_{11} - $ \texttt{BlockMatrixProduct}($L_{10}, U_{01}$))
    \State $L \gets [L_{00}, 0; L_{10}, L_{11}]$
    \State $U \gets [U_{00}, U_{01}; 0, U_{11}]$
\EndIf
\Comment{$L$ and $U$ have the same block structure as $C$}
\State \textbf{return} $\gets [L, U]$
\end{algorithmic}
\end{algorithm}

==> codes/blockproduct.tex <==
\begin{algorithm}[t]
\caption{\texttt{BlockMatrixProduct}($A, B$)}\label{alg:blockproduct}

\begin{algorithmic}
\Ensure $A, B$ hierarchical matrices with same index-tree $T$
\State $C \gets \emptyset$  
\Comment{hierarchical matrix}
\If{$A, B$ leafs in $T$}
    \If{$A, B$ low-rank}
        \Comment{ $A = S_A T_A^{\intercal} , B = S_B T_B^{\intercal}$}
        \State $C \gets (S_A T_A^{\intercal}S_B) \cdot T_B^{\intercal}$
    \Else 
        \Comment{store as low-rank}
        \State $C \gets A \cdot B$
    \EndIf
    \Comment{store as dense}
\Else 
    \State $[A_{00}, A_{01}; A_{10}, A_{11}] \gets A$
    \Comment{with respect to $T$}
    \State $[B_{00}, B_{01}; B_{10}, B_{11}] \gets B$
    \ForEach{$(A_{ik}, B_{kj})$}
        \State $C_{ij} \gets C_{ij} + $ \texttt{BlockMatrixProduct}$(A_{ik}, B_{kj})$
    \EndFor
    \State $C \gets [C_{00}, C_{01}; C_{10}, C_{11}]$
    \Comment{preserving hierarchical structure}
\EndIf
\end{algorithmic}
\end{algorithm}
